OpenKBP-Opt: An international and reproducible evaluation of 76 knowledge-based planning pipelines

We establish an open framework for developing plan optimization models for knowledge-based planning (KBP) in radiotherapy. Our framework includes reference plans for 100 patients with head-and-neck cancer and high-quality dose predictions from 19 KBP models that were developed by different research groups during the OpenKBP Grand Challenge. The dose predictions were input to four optimization models to form 76 unique KBP pipelines that generated 7600 plans. The predictions and plans were compared to the reference plans via: dose score, which is the average mean absolute voxel-by-voxel difference in dose a model achieved; the deviation in dose-volume histogram (DVH) criterion; and the frequency of clinical planning criteria satisfaction. We also performed a theoretical investigation to justify our dose mimicking models. The range in rank order correlation of the dose score between predictions and their KBP pipelines was 0.50 to 0.62, which indicates that the quality of the predictions is generally positively correlated with the quality of the plans. Additionally, compared to the input predictions, the KBP-generated plans performed significantly better (P<0.05; one-sided Wilcoxon test) on 18 of 23 DVH criteria. Similarly, each optimization model generated plans that satisfied a higher percentage of criteria than the reference plans. Lastly, our theoretical investigation demonstrated that the dose mimicking models generated plans that are also optimal for a conventional planning model. This was the largest international effort to date for evaluating the combination of KBP prediction and optimization models. In the interest of reproducibility, our data and code is freely available at https://github.com/ababier/open-kbp-opt.

==> results/criteria.tex <==
\begin{tabular}{llllllll}
\toprule
Dose_type & Reference & Prediction &         MeanAbs & MaxAbs &         MeanRel & MaxRel &            Best \\
\midrule
Brainstem     &      96.6 &       97.3 &  \textbf{100.0} &   99.5 &  \textbf{100.0} &   98.5 &  \textbf{100.0} \\
Spinal cord   &      95.5 &       92.7 &            99.7 &   97.3 &  \textbf{100.0} &   95.6 &  \textbf{100.0} \\
Right parotid &      32.3 &       32.7 &   \textbf{46.1} &   38.9 &            45.0 &   38.0 &            41.4 \\
Left parotid  &      30.6 &       30.1 &   \textbf{43.7} &   35.0 &            41.9 &   35.0 &            40.8 \\
Esophagus     &      93.0 &       92.7 &  \textbf{100.0} &   95.2 &  \textbf{100.0} &   97.3 &  \textbf{100.0} \\
Larynx        &      37.7 &       34.7 &   \textbf{71.5} &   44.9 &            58.8 &   44.6 &            67.9 \\
Mandible      &      87.5 &       89.4 &   \textbf{99.6} &   98.7 &            99.2 &   99.0 &            93.1 \\
PTV56         &      91.2 &       85.8 &            83.3 &   91.8 &            84.1 &   84.6 &   \textbf{96.7} \\
PTV63         &      90.5 &       86.2 &            82.2 &   89.6 &            84.8 &   84.8 &   \textbf{92.9} \\
PTV70         &      64.0 &       45.7 &            37.2 &   51.6 &            40.1 &   47.7 &   \textbf{66.0} \\
OARs          &      65.5 &       65.1 &   \textbf{77.1} &   70.6 &            75.3 &   70.2 &            74.5 \\
Targets       &      79.4 &       68.7 &            63.3 &   74.2 &            65.3 &   68.8 &   \textbf{82.8} \\
All ROIs      &      69.7 &       66.2 &            72.9 &   71.7 &            72.3 &   69.8 &   \textbf{77.0} \\
\bottomrule
\end{tabular}


==> results/optimization_meta_data.tex <==
\begin{tabular}{lllll}
\toprule
{} & MeanAbs & MaxAbs & MeanRel & MaxRel \\
\midrule
OARs                      &   0.018 &  0.011 &   0.554 &  0.417 \\
Optimization              &   0.006 &  0.170 &   0.028 &  0.014 \\
Targets                   &   0.976 &  0.819 &   0.418 &  0.569 \\
Mean solve time           &     389 &    222 &     367 &    393 \\
First quartile solve time &     192 &    107 &     183 &    188 \\
Third quartile solve time &     502 &    261 &     481 &    507 \\
\bottomrule
\end{tabular}

